Effect of Homomorphic Encryption on the Performance of Training Federated Learning Generative Adversarial Networks

A Generative Adversarial Network (GAN) is a deep-learning generative model in the field of Machine Learning (ML) that involves training two Neural Networks (NN) using a sizable data set. In certain fields, such as medicine, the training data may be hospital patient records that are stored across different hospitals. The classic centralized approach would involve sending the data to a centralized server where the model would be trained. However, that would involve breaching the privacy and confidentiality of the patients and their data, which would be unacceptable. Therefore, Federated Learning (FL), an ML technique that trains ML models in a distributed setting without data ever leaving the host device, would be a better alternative to the centralized option. In this ML technique, only parameters and certain metadata would be communicated. In spite of that, there still exist attacks that can infer user data using the parameters and metadata. A fully privacy-preserving solution involves homomorphically encrypting (HE) the data communicated. This paper will focus on the performance loss of training an FL-GAN with three different types of Homomorphic Encryption: Partial Homomorphic Encryption (PHE), Somewhat Homomorphic Encryption (SHE), and Fully Homomorphic Encryption (FHE). We will also test the performance loss of Multi-Party Computations (MPC), as it has homomorphic properties. The performances will be compared to the performance of training an FL-GAN without encryption as well. Our experiments show that the more complex the encryption method is, the longer it takes, with the extra time taken for HE is quite significant in comparison to the base case of FL.

==> sections/responsible_research.tex <==
\section{Responsible Research}
While initially studying and reading through research papers and articles, an effort was made to ensure the papers were written by different authors performing their research from different parts of the world. That was done to ensure our starting point was as unbiased as possible, and our knowledge diverse to the greatest extent. All of the resources used are publicly available, and can be accessed by anyone. Moreover, we have attempted to explore technologies developed by industry standard companies, such as Facebook/Meta and Google. We believed studying the work of such reputable companies would decrease the probability of any bias being included in the research. They have the resources and responsibility to ensure their work is at the highest possible level. 

Furthermore, there was no personal bias involved when implementing the FL-GAN with HE. Our sole objective was to study the effect of HE on the performance of training such ML models. We used the most famous tool we could find, which were all open source. We also went over a considerable amount of repositories that we attempted to use unsuccessfully, which can be recreated by anyone. We also thought that including it in the paper would save any future research valuable time when trying to solve a similar problem.

Lastly, while our study focuses on the impact of the performance loss of using HE on FL-GANs, the whole idea of using HE is to increase the privacy of the end users. That is a hot topic in today's world, and motivates us to be extra delicate and careful to ensure the most accurate results and implementations. While our implementation is not 100\% real world applicable and is more research based, we hope that it may be helpful with creating an implementation that is.
